Mixed-precision algorithms for solving the Sylvester matrix equation

We consider the solution of the Sylvester equation $AX+XB=C$ in mixed precision. We derive a new iterative refinement scheme to solve perturbed quasi-triangular Sylvester equations; our rounding error analysis provides sufficient conditions for convergence and a bound on the attainable relative residual. We leverage this iterative scheme to solve the general Sylvester equation. The new algorithms compute the Schur decomposition of the coefficient matrices $A$ and $B$ in lower than working precision, use the low-precision Schur factors to obtain an approximate solution to the perturbed quasi-triangular equation, and iteratively refine it to obtain a working-precision solution. In order to solve the original equation to working precision, the unitary Schur factors of the coefficient matrices must be unitary to working precision, but this is not the case if the Schur decomposition is computed in low precision. We propose two effective approaches to address this: one is based on re-orthonormalization in working precision, and the other on explicit inversion of the almost-unitary factors. The two mixed-precision algorithms thus obtained are tested on various Sylvester and Lyapunov equations from the literature. Our numerical experiments show that, for both types of equations, the new algorithms are at least as accurate as existing ones. Our cost analysis, on the other hand, suggests that they would typically be faster than mono-precision alternatives if implemented on hardware that natively supports low precision.

==> figs/cost_ratio.tex <==
\pgfplotscreateplotcyclelist{iterlist}{
  mark=none, draw=BrickRed\\
  mark=none, draw=PineGreen\\
  only marks, mark=asterisk, draw=RoyalBlue, mark repeat=4, mark phase=2, line width=0.9pt, \\
  mark=none, draw=BrickRed, densely dashed\\
}

\newcommand{\drawplotcost}[2]{
  \begin{tikzpicture}[trim axis right, trim axis left]
    \begin{axis}[
      width = 0.42\textwidth,
      height = 0.34\textwidth,
      xmin = 0, xmax = 1,
      ymin = 0.3, ymax = 1.4,
      xlabel={$\rho$},
      legend pos=south west,
      mark size= 4pt,
      line width=1.8pt,
      cycle list name = iterlist
      ]

      \addplot table[x=rho, y=cost_stit_#1]{\mydata};
      \addplot table[x=rho, y=cost_stit_#2]{\mydata};

    \end{axis}
  \end{tikzpicture}}


\begin{figure}[t!]
  \setlength\figwidth{0.42\linewidth}
  \pgfplotstableread{figs/cost_ratio.dat}\mydata
  \centering
  \subfigure[Sylvester equations.]{
    \label{fig:cost-a}
    \drawplotcost{sylv_orth}{sylv_inv}}\hspace{30pt}
  \subfigure[Lyapunov equations.]{
    \label{fig:cost-b}
    \drawplotcost{lyap_orth}{lyap_inv}}\\
  \caption{Cost ratio of the mixed-precision iterative refinement algorithms over the Bartels--Stewart algorithm run in high precision when $k=0$.}
  \label{fig:cost-ratio}
\end{figure}


==> figs/optk-funk-old.tex <==

\newcommand{\drawplotcombined}[1]{
\begin{tikzpicture}[trim axis right, trim axis left]
  \begin{axis}[
    width=0.42\textwidth,
    height=0.34\textwidth,
    scale only axis,
    xmin=0, xmax=1,
    ymin=-3, ymax=8,
    xlabel={$\rho$},
    mark size=4pt,
    line width=1.8pt,
  ]
    \addplot[
      mark=*,
      only marks,
      draw opacity=0,
      fill=JungleGreen!40,
      line width=0.9pt,
      mark repeat=4,
      mark phase=2
    ] table[x=rho, y={optk_stit_#1}] {\dataoptk};

    \addplot[
      mark=none,
      line width=1.8pt,
      draw=PineGreen
    ] table[x=rho, y={funk_stit_#1}] {\dataoptk};
  \end{axis}


\end{tikzpicture}
}

\newcommand{\makelegendcombined}{
  \begin{tikzpicture}
    \begin{axis}[
      legend columns=3,
      scale only axis,
      width=1mm,
      legend style={
        inner sep=6pt,
        column sep=30pt,
        cells={mark size=4pt, line width=1.8pt},
        legend cell align=left,
        at={(0,0)},
        anchor=center,
        draw=none
      }
    ]
      \addplot[
        mark=*,
        only marks,
        draw opacity=0,
        fill=JungleGreen!40,
        line width=0.9pt,
        mark repeat=4,
        mark phase=2
      ] coordinates {(0,0) (1,0)};
      \addlegendentry{$\optk$ in~\eqref{eq:optk}}

      \addplot[
        mark=none,
        draw=PineGreen
      ] coordinates {(0,0) (1,0)};
      \addlegendentry{$\funk$}

    \end{axis}
  \end{tikzpicture}
}

\begin{figure}[t!]
  \pgfplotstableread{figs/optk.dat}\dataoptk
  \pgfplotstableread{figs/cost_ratio.dat}\datacost
  \centering

  \subfigure[Algorithm~\ref{alg:sylv-mp} for Sylvester equations.]{
    \label{fig:optk-a}
    \drawplotcombined{sylv_orth}}\hspace{30pt}
  \subfigure[Algorithm~\ref{alg:sylv-mp} for Lyapunov equations.]{
    \label{fig:optk-b}
    \drawplotcombined{lyap_orth}}\\

  \subfigure[Algorithm~\ref{alg:sylv-mp-inversion} for Sylvester equations.]{
    \label{fig:optk-c}
    \drawplotcombined{sylv_inv}}\hspace{30pt}
  \subfigure[Algorithm~\ref{alg:sylv-mp-inversion} for Lyapunov equations.]{
    \label{fig:optk-d}
    \drawplotcombined{lyap_inv}}\\

  \subfigure[Legend]{\makelegendcombined}

  \caption{Maximum number of iterations for which the iterative refinement algorithms in Section~\ref{sec:pert-sylv-algs} will be asymptotically faster than the Bartels--Stewart algorithm run in high precision (left axis),
  where we are plotting the quantities in~\eqref{eq:funk-orth},~\eqref{eq:funk-orth-lyap},~\eqref{eq:funk-inv}, and~\eqref{eq:funk-inv-lyap} against the ratio $\ratio$ of the computational cost of low-precision to a high-precision operation.
  Also shown is the cost ratio of mixed-precision iterative refinement to high-precision Bartels--Stewart for $i=1$ (right axis).}
  \label{fig:optk}
\end{figure}

